Random Generation of $k$-coloured Motzkin Paths

We study k-coloured Motzkin paths, namely Motzkin paths in which horizontal steps can be coloured in k different ways, and investigate their connection with the number of prefixes ending at odd height from both an analytical and a combinatorial point of view. Moreover, the combinatorial approach provides a random generation algorithm for k-coloured Motzkin paths in linear-time.

==> eptcsdata.tex <==
\providecommand{\firstpage}{10}
\providecommand{\publicationstatus}{S. Brlek and L. Ferrari (Eds.): GASCom 2026\\
EPTCS 445, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.445.2}{10.4204/EPTCS.445.2}}
\pdfoutput=1

